PIVETed-Granite: Computational Phenotypes through Constrained Tensor Factorization

It has been recently shown that sparse, nonnegative tensor factorization of multi-modal electronic health record data is a promising approach to high-throughput computational phenotyping. However, such approaches typically do not leverage available domain knowledge while extracting the phenotypes; hence, some of the suggested phenotypes may not map well to clinical concepts or may be very similar to other suggested phenotypes. To address these issues, we present a novel, automatic approach called PIVETed-Granite that mines existing biomedical literature (PubMed) to obtain cannot-link constraints that are then used as side-information during a tensor-factorization based computational phenotyping process. The resulting improvements are clearly observed in experiments using a large dataset from VUMC to identify phenotypes for hypertensive patients.

==> sections/background_v3.tex <==

%\small{
%\begin{table*}[]
%\centering
%\caption{Phenotypes most associated with patients who were diagnosed with at least one myocardial infarction.}
%\label{tab:phenos}
%\begin{tabular}{llll|l|}
%\cline{1-1} \cline{3-3} \cline{5-5}
%\multicolumn{1}{|l|}{\textbf{Phenotype 10}}                                           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Phenotype 11}}                                        &  & \textbf{Phenotype 28}                                                                                                    \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{\textit{23.67\% total patients (40.26\% AMI patients)}}          & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textit{23.67\% total patients (33.77\% AMI patients)}}       &  & \textit{17.94\% total patients (35.06\% AMI patients)}                                                                   \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{3531FF} Hypertensive chronic kidney disease}}      & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{3531FF} Chronic renal failure {[}CKD{]}}}       &  & {\color[HTML]{3531FF} Nonspecific chest pain}                                                                            \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{3531FF} Congestive heart failure (CHF) NOS}}       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{3531FF} Essential hypertension}}                &  & {\color[HTML]{3531FF} Type 2 diabetes}                                                                                   \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{3531FF} Nonspecific chest pain}}                   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{F56B00} diuretics}}                             &  & {\color[HTML]{3531FF} Coronary atherosclerosis}                                                                          \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} diuretics}}                                & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{F56B00} glucose elevating agents}}              &  & {\color[HTML]{3531FF} Disturbance of skin sensation}                                                                     \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} angiotensin converting enzyme inhibitors}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{F56B00} antihyperlipidemic agents}}             &  & {\color[HTML]{3531FF} \begin{tabular}[c]{@{}l@{}}Agorophobia, social phobia,\\          and panic disorder\end{tabular}} \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} antihyperlipidemic agents}}                &                       &                                                                                   &  & {\color[HTML]{3531FF} Fever of unknown origin}                                                                           \\ \cline{1-1} \cline{5-5} 
%                                                                                      &                       &                                                                                   &  & {\color[HTML]{3531FF} Other paralytic syndromes}                                                                         \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{\textbf{Phenotype 16}}                                           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Phenotype 21}}                                        &  & {\color[HTML]{3531FF} Constipation}                                                                                      \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{\textit{19.73\% total patients (28.57\% AMI patients)}}          & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textit{25.28\% total patients (28.57\% AMI patients)}}       &  & {\color[HTML]{3531FF} Gastrojejunal ulcer}                                                                               \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{3531FF} Atrial fibrillation}}                      & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{3531FF} Type 2 diabetes}}                       &  & {\color[HTML]{F56B00} analgesics}                                                                                        \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{3531FF} Essential hypertension}}                   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{F56B00} antiarrhythmic agents}}                 &  & {\color[HTML]{F56B00} mouth and throat products}                                                                         \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} calcium channel blocking agents}}          & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{\color[HTML]{F56B00} anxiolytics, sedatives, and hypnotics}} &  & {\color[HTML]{F56B00} proton pump inhibitors}                                                                            \\ \cline{1-1} \cline{3-3} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} adrenal cortical steroids}}                &                       &                                                                                   &  & {\color[HTML]{F56B00} calcium channel blocking agents}                                                                   \\ \cline{1-1} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} antiarrhythmic agents}}                    &                       &                                                                                   &  & {\color[HTML]{F56B00} antidepressants}                                                                                   \\ \cline{1-1} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} diuretics}}                                &                       &                                                                                   &  & {\color[HTML]{F56B00} antiseptic and germicides}                                                                         \\ \cline{1-1} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} nasal preparations}}                       &                       &                                                                                   &  & {\color[HTML]{F56B00} smoking cessation agents}                                                                          \\ \cline{1-1} \cline{5-5} 
%\multicolumn{1}{|l|}{{\color[HTML]{F56B00} inotropic agents}}                         &                       &                                                                                   &  & {\color[HTML]{F56B00} vasodilators}                                                                                      \\ \cline{1-1} \cline{5-5} 
%\end{tabular}
%\end{table*}}

%\section{Background}
%We briefly describe tensors and the process of decomposing them but refer the reader to~\cite{Kolda:2009dh} for a more detailed account.
%A tensor is an $n$-way or $n$-mode array that is used to represent $n$-dimensional relationships.
%%In this work, we focus on $3$-mode tensors where patients, diagnoses, and medications form the three modes.
%%Each element of a tensor captures the multidimensional relationship of the number of times a patient received a diagnosis and medication prescription in a given period of time.
%We use CANDECOMP / PARAFAC (CP) decomposition \cite{Harshman:1970vk} to factor the tensor.
%For a tensor $\TX{X}$ with $N$ modes, the CP decomposition is
%\begin{align}
%\TX{X} &\approx \displaystyle \sum_{r=1}^R \lambda_r \M{a}_r^{(1)} \op \hdots \op \M{a}_r^{(N)} = \llbracket \BS{\lambda}; \FN{A}{1}; \hdots; \FN{A}{N} \rrbracket,.
%\end{align}
%where each component of the sum is a rank-one tensor formed by taking the outer product of N vectors, $\FN{a}{1} \op \FN{a}{2} \op \cdots \op \FN{a}{N}$.
%The representation $\llbracket \BS{\lambda}; \FN{A}{1}; \hdots; \FN{A}{N} \rrbracket$ is shorthand notation with the weight vector $\BS{\lambda} = [\lambda_1 \cdots \lambda_R]$ and the factor matrix $\M{A}^{(n)} = [\FN{a}{n}_1 \cdots \FN{a}{n}_R],$ where $\M{a}_r$  denotes the \nth{r} column of $\M{A}^{(n)}$.
%CP decompositions are usually fit using a loss function that makes assumptions about the underlying distribution that generated the data in the tensor (e.g., Gaussian or Poisson).
%%In general, tensor factorization utilizes information in the multiway structure to produce factors that are more concise and potentially more interpretable than the original data~\cite{Kolda:2009dh}.
%When CP decomposition is applied to Electronic Health Records (EHRs), each rank one tensor can be thought of a candidate phenotypes that must be evaluated as clinically relevant or not.

%Carroll:1970tm,

%Standard CP decomposition is formulated as a least squares approximation (data follows a Gaussian distribution), which makes it well-suited for continuous data. 
%This also results in simpler algorithms, and the ADMM technique can be readily applied for distributed computation.



